Electroweak Contributions to Thermal Gravitino Production

At high temperatures, gravitinos are generated in inelastic scattering processes with particles that are in thermal equilibrium with the hot primordial plasma. We consider the regeneration of gravitinos that starts with completion of reheating after inflation. Following a consistent finite-temperature approach, we provide the complete result for the gravitino production rate to leading order in the gauge couplings. Focusing on gravitino dark matter scenarios we compute the relic density of thermally produced gravitinos. Moreover, we show that a conceivable determination of the gravitino mass at future colliders will allow for a unique test of the viability of thermal leptogenesis in the laboratory.

==> gdm.tex <==

\chapter{Gravitino Dark Matter}
\label{cha:grav-dark-matt}



%
%
%
%
%
%
%




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "thesis"
%%% End: 

